ProofBuddy: How it Started, How it's Going

We report on our journey to develop ProofBuddy, a web application that is powered by a server-side instance of the proof assistant Isabelle, for the teaching and learning of proofs and proving. The journey started from an attempt to use just Isabelle in an educational context. Along the way, following the educational design research approach with a series of experiments and their evaluations, we observed that a web application like \ProofBuddy has many advantages over a desktop application, for developers and teachers as well as for students. In summary, the advantages cover simplicity, maintainability and customizability. We particularly highlight the latter by exhibiting the potential of interactive tutorials and their implementation within ProofBuddy.

==> eptcsdata.tex <==
\providecommand{\firstpage}{90}
\providecommand{\publicationstatus}{J. Narboux, W. Neuper and P. Quaresma (Eds.): Theorem Proving\\ Components for Educational Software 2024 (ThEdu'24)\\
EPTCS 419, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.419.6}{10.4204/EPTCS.419.6}}
\pdfoutput=1

